No-Free-Graph: Learning When Multimodal Data Should Be Graphified

Multimodal graph learning has recently emerged as an effective paradigm for in corporating inter-entity relationships into multimodal representations. Existing studies have made substantial progress on how to construct and optimize graphs, but rarely consider a more fundamental question: whether additional relational structures should be introduced for a given dataset and task. Through empirical studies across diverse datasets, tasks, and graph constructors, we reveal that graphification is not consistently beneficial: introducing relational structures can provide substantial improvements in some cases, while offering limited or even negative gains. This observation motivates a new perspective that graph construction should be treated as a selective decision based on its expected utility rather than a default preprocessing step. To address this issue, we propose MAG-SCOUT, a pre-construction graph assessment framework that estimates whether introducing graph structures is beneficial before generating the complete topology. MAG-SCOUT collects limited relational evidence, analyzes its potential taskspecific contribution, and estimates the expected utility of graphification together with construction cost to make a build-or-skip decision. Extensive experiments across six multimodal datasets, three downstream tasks, and diverse graph constructors demonstrate that MAG-SCOUT effectively identifies when graph structures should be introduced, saving 33.1% of task-macro graph work while retaining 96.7% of held-out positive-gain mass under the pre-registered floor.

==> tables/q3_operating_points.tex <==
\begin{table}[!htbp]
\centering
\definecolor{magL}{HTML}{EAF2FB}
\caption{Q3 policy outcomes at nested validation-selected thresholds across 13 parent sources. Saved graph work and retention are task-macro quantities. An asterisk ($^*$) marks a held-out value below the 95\% retention floor. Always-Build and Oracle are references.}
\label{tab:q3-operating-points}
\scriptsize
\setlength{\tabcolsep}{5pt}
\renewcommand{\arraystretch}{1.22}
\resizebox{\textwidth}{!}{%
\begin{tabular}{@{}l !{\vrule width 0.7pt} c !{\vrule width 0.5pt} c !{\vrule width 0.5pt} c !{\vrule width 0.7pt} c@{}}
\toprule[1.2pt]
\BoldLabel{Policy / Predictor} & \BoldLabel{Saved Graph Work (\%)} $\uparrow$ & \BoldLabel{Retained Gain Mass (\%)} $\uparrow$ & \BoldLabel{Wrong Skip (\%)} $\downarrow$ & \BoldLabel{Build Rate (\%)} $\downarrow$ \\
\midrule[0.7pt]
\rowcolor{magL}\BoldLabel{MAG-Scout (Ours)} & 23.6 & \textbf{96.7} & 13.3 & 76.7 \\
\BoldLabel{NetInfoF} & 23.2 & \underline{96.4} & \textbf{9.3} & 76.9 \\
\BoldLabel{WDGH} & 23.5 & 90.5$^*$ & \underline{10.1} & 76.5 \\
\BoldLabel{GLEMOS-S2} & \underline{30.3} & 60.5$^*$ & 25.5 & \underline{70.8} \\
\BoldLabel{MetaGL} & \textbf{32.6} & 80.2$^*$ & 27.7 & \textbf{68.7} \\
\midrule[0.5pt]
Always Build & \textcolor{gray}{0.0} & \textcolor{gray}{100.0} & \textcolor{gray}{0.0} & \textcolor{gray}{100.0} \\
Oracle (Unattainable Bound) & \textcolor{gray}{57.7} & \textcolor{gray}{100.0} & \textcolor{gray}{0.0} & \textcolor{gray}{42.9} \\
\bottomrule[1.2pt]
\end{tabular}%
}
\par\vspace{3pt}
{\scriptsize Task-macro scores average source-level ratios within NC, LP, and CMR, then average the three tasks. Saved graph work is the fraction of graphification cost avoided relative to Always-Build. \textbf{MAG-Scout} and NetInfoF meet the 95\% floor. Their paired parent-source bootstrap saved-work difference is \QThreeNetInfoSavedDiff points (95\% CI $[\QThreeNetInfoSavedCILow,\ \QThreeNetInfoSavedCIHigh]$); it need not equal the subtraction of the rounded headline values.}
\end{table}

